Residual Policy Gradient: A Reward View of KL-regularized Objective

Reinforcement Learning and Imitation Learning have achieved widespread success in many domains but remain constrained during real-world deployment. One of the main issues is the additional requirements that were not considered during training. To address this challenge, policy customization has been introduced, aiming to adapt a prior policy while preserving its inherent properties and meeting new task-specific requirements. A principled approach to policy customization is Residual Q-Learning (RQL), which formulates the problem as a Markov Decision Process (MDP) and derives a family of value-based learning algorithms. However, RQL has not yet been applied to policy gradient methods, which restricts its applicability, especially in tasks where policy gradient has already proven more effective. In this work, we first derive a concise form of Soft Policy Gradient as a preliminary. Building on this, we introduce Residual Policy Gradient (RPG), which extends RQL to policy gradient methods, allowing policy customization in gradient-based RL settings. With the view of RPG, we rethink the KL-regularized objective widely used in RL fine-tuning. We show that under certain assumptions, KL-regularized objective leads to a maximum-entropy policy that balances the inherent properties and task-specific requirements on a reward-level. Our experiments in MuJoCo demonstrate the effectiveness of Soft Policy Gradient and Residual Policy Gradient.

==> chap5_RLC2025.tex <==
\chapter{Residual Policy Gradient: A Reward View of KL-regularized Objective}
\label{chap:rlc2025}
% Policy Customization is important
Reinforcement Learning and Imitation Learning have achieved widespread success in many domains but remain constrained during real-world deployment. One of the main issues is the additional requirements that were not considered during training.
% Definition of Policy Customization
To address this challenge, policy customization has been introduced, aiming to adapt a prior policy while preserving its inherent properties and meeting new task-specific requirements. 
% RQL can solve that
A principled approach to policy customization is Residual Q-learning (RQL), which formulates the problem as a Markov Decision Process (MDP) and derives a family of value-based learning algorithms. 
% it is not enough
However, RQL has not yet been applied to policy gradient methods, which restricts its applicability, especially in tasks where policy gradient has already proven more effective. 
% Contribution 1:
In this chapter, we first derive a concise form of \emph{Soft Policy Gradient} as a preliminary. 
% Contribution 2:
Building on this, we introduce \emph{Residual Policy Gradient} (RPG), which extends RQL to policy gradient methods, allowing policy customization in gradient-based RL settings.
% Contribution 3:
With the view of RPG, we rethink the KL-regularized objective widely used in RL fine-tuning. We show that under certain assumptions, KL-regularized objective leads to a maximum-entropy policy that balances the inherent properties and task-specific requirements on thr reward-level.
% Experiments
Our experiments in MuJoCo demonstrate the effectiveness of \emph{Soft Policy Gradient} and \emph{Residual Policy Gradient}.

\newpage
\section{Introduction}\label{sec:RLC-intro}

%%% Policy Customization is Important
% General Policy Learning
Policy learning algorithms, such as Reinforcement Learning (RL) and Imitation Learning (IL), have achieved great success across various cross-domain tasks, including locomotion~\parencite{liang2024adaptive}, autonomous racing~\parencite{Sophy}, and Large Language Model (LLM)~\parencite{guo2025deepseek}. 
% Additional Requirements
However, practical deployments often impose additional requirements on the trained policies beyond those established during training, such as configuring the robot-human hand-over~\parencite{cakmak2011human} or membership behaviour~\parencite{correia2019choose} with preferences. 
% % Policy Customization is essential to meet this need
% Under this context, retraining a policy network from scratch for each new objective can be both costly and inefficient. 
% Policy Customization introduction
To elaborate the challenge, \textit{policy customization}, introduced in the previous chapter, aims to modify a prior policy, ensuring that the new policy (1) retains properties of the original and (2) adapts to new task-specific requirements.


% RQL Introduction and Policy Gradients Limitation 1
Residual Q-learning (RQL) provides a principled approach to policy customization by formulating the problem as a Markov Decision Process (MDP), which jointly optimizes the reward of the prior and the add-on task-specified reward. It derives a theoretical learning objective through the Q-function and provides a family of practical learning and planning algorithms.
% However, it has primarily been applied in value-based RL and has not yet been extended to policy gradient methods, a fundamental class of algorithms in modern reinforcement learning.
% % Example
% This limitation restricts the applicability of RQL, especially when large-scale parallel environments are available, policy gradient methods tend to outperform value-based methods~\parencite{gallici2024simplifying}.
However, it has primarily been applied in value-based RL and has not yet been extended to policy gradient methods, a fundamental class of algorithms in modern reinforcement learning, which restricts the applicability of RQL.
% Example
This limitation becomes more pronounced when large-scale parallel environments are available, where policy gradient methods tend to outperform value-based methods~\parencite{gallici2024simplifying}.
% So it is important
Therefore, it is of great importance to derive the policy gradient extension of RQL.
% Contribution1&2: Soft PPO & Residual PPO

% Soft Policy Gradient
In this chapter, we first derive a concise form of maximum-entropy policy gradient method, \emph{Soft Policy Gradient}, as the preliminary method and compare it with similar forms in the related literature.
% Residual Policy Gradient
Based on the derived form, we further propose \emph{Residual Policy Gradient} (RPG) to solve the policy customization using a policy gradient approach. Our experiments in MuJoCo demonstrate the effectiveness of \emph{Soft Policy Gradient} and \emph{Residual Policy Gradient}.
% KL
Moreover, from the perspective of RPG, we rethink the widely used KL-regularized objective in RL fine-tuning. We show that:
(1) If the prior policy models an optimal Bolzmann distribution, the KL-regularized objective induces a maximum-entropy policy that balances inherent properties and task-specific requirements at the reward level.
(2) This formulation can be further refined through a simple decoupling, leading to improved optimization efficiency.
% RLHF example
In Appendix~\ref{appendix:RLC-RLHF}, we elaborate these insights with RL-based LLM fine-tuning, demonstrating their implications for both theoretical understanding and future research directions.



\section{Preliminaries}\label{sec:RLC-Preliminaries}
In this section, we introduce two techniques mainly used in the proposed algorithms, Policy Gradient and RQL, laying the foundation for the subsequent derivations and analysis. 


\subsection{Policy Gradient Method}\label{sec:RLC-PG}

Policy gradient methods are one of the largest families of RL algorithms, which directly optimizes the policy $\pi_\theta$ on the expected return $J$ of a discounted reward function $r$ by estimating its gradient:

\begin{equation}\label{eqn:PG obj}
\nabla_\theta J(\pi_\theta) = \nabla_\theta \mathbb{E}_{(\boldsymbol{s}_t,\boldsymbol{a}_t)\sim\pi_\theta,p(\cdot|\boldsymbol{s},\boldsymbol{a})}\left[\sum_{t=0} \gamma^t \left(r(\boldsymbol{s}_t,\boldsymbol{a}_t)\right)\right],
\end{equation}

where $\gamma$ is the discounted factor, and $p(\cdot|\boldsymbol{s},\boldsymbol{a})$ is the transition probability of the environment. Based on Eqn.~(\ref{eqn:PG obj}), various practical algorithms have been developed to effectively address a wide range of tasks. A typical example is PPO~\parencite{schulman2017proximal}, which ensures stable and reliable updates by introducing a clipped objective function:

\begin{equation}\label{eqn:PPO obj}
\quad \nabla_\theta J(\pi_\theta) = \nabla_\theta \mathbb{E}_{(\boldsymbol{s}_t,\boldsymbol{a}_t)\sim\pi_\theta,p(\cdot|\boldsymbol{s},\boldsymbol{a})} \left[ \min \{r_t(\pi_\theta) A_t, \operatorname{clip}(r_t(\pi_\theta), 1 - \epsilon, 1 + \epsilon) A_t \} \right],
\end{equation}
where $r_t(\pi_\theta) = \frac{\pi_\theta(\boldsymbol{a}_t | \boldsymbol{s}_t)}{\pi_{\theta_{old}}(\boldsymbol{a}_t | \boldsymbol{s}_t)}$ denotes the probability ratio, $A_t$ is the estimator of the advantage function at timestep t, and $\epsilon$ is a hyperparameter. This augmented form limits policy updates within a pre-defined range, balancing exploration and exploitation without complex constraints.



\subsection{Policy Customization and Residual Q-Learning}\label{sec:RLC-RQL}
% The goal of policy customization is to derive a policy from a prior policy that satisfies the new requirements of an add-on task while maintaining the performance of the original task. Thus, it is assumed that a well-trained prior policy is available for policy customization. 
Consider a MDP defined by $\mathcal{M} = (\mathcal{S}, \mathcal{A}, r, p)$, where $\mathcal{S}$ and $\mathcal{A}$ are state and action spaces, $r$ is the reward function, and $p$ is the transition probability density function. The objective of policy customization is to derive a new policy that optimally solves a modified MDP, $\hat{\mathcal{M}} = (\mathcal{S}, \mathcal{A}, \omega r+r_R, p)$, where $r_R$ is the add-on task-specified reward and $\omega$ is the weight parameter. In particular, policy customization is especially relevant in scenarios where the basic reward $r$ is unknown, but a prior policy $\pi$, trained as an optimal maximum-entropy policy for $\mathcal{M}$, is available.

The previous chapter proposes the residual Q-learning (RQL) framework to solve the policy customization. 
Given the prior policy $\pi$, RQL is able to find this customized policy without the reward knowledge of the prior policy $r$, which ensures broader applicability across different prior policies obtained through various methods, including those solely imitating demonstrations. Specifically, by defining the Residual Q function $Q_R = \hat{Q} - \omega Q^*$, where $Q^*$ and $\hat{Q}$ are the optimal value function on $\mathcal{M}$ and the updating value function on $\hat{\mathcal{M}}$, RQL updates the $Q_R$ using the following equation:
\begin{equation}
\label{eqn:RLC-RQL}
    Q_R(\boldsymbol{s}, \boldsymbol{a}) \leftarrow r_R(\boldsymbol{s}, \boldsymbol{a}) + \gamma \mathbb{E}_{s'}\left[\hat{\alpha}\log \int_{\mathcal{A}}\exp\left(\frac{1}{\hat{\alpha}}\left({Q}_{R} (\boldsymbol{s}', \boldsymbol{a}')+\omega\alpha\log \pi\left(\boldsymbol{a}' \vert \boldsymbol{s}'\right)\right)\right)d\boldsymbol{a}'\right],
\end{equation}
where $\alpha$ and $\hat{\alpha}$ are the entropy-encouragement coefficients of maximum-entropy policy on prior and full task, and $\gamma$ is the discounted factor.
As shown in the RQL appendix, by adding $\omega \alpha \log \pi\left(\boldsymbol{a}_{t}| \boldsymbol{s}_{t}\right)$ to both sides of Eqn.~(\ref{eqn:RLC-RQL}) and defining $Q^\text{aug}_R\left(\boldsymbol{s}, \boldsymbol{a}\right) = Q_R\left(\boldsymbol{s}, \boldsymbol{a}\right) + \omega\alpha\log \pi\left(\boldsymbol{a} \vert \boldsymbol{s}\right)$, we can reformulate Eqn.~(\ref{eqn:RLC-RQL}) as:
\begin{equation}
\label{eqn:RLC-RQL_aug}
   Q^\text{aug}_R(\boldsymbol{s}, \boldsymbol{a}) \leftarrow r_R(\boldsymbol{s}, \boldsymbol{a}) + \omega\alpha\log \pi\left(\boldsymbol{a} \vert \boldsymbol{s}\right) + \gamma \mathbb{E}_{s'}\left[\hat{\alpha}\log \int_{\mathcal{A}}\exp\left(\frac{1}{\hat{\alpha}}{Q}^\text{aug}_R (\boldsymbol{s}', \boldsymbol{a}')\right)d\boldsymbol{a}'\right],
\end{equation}
which is a standard soft-Q update on an augmented MDP problem, $$\mathcal{M}^\mathrm{aug} = (\mathcal{S}, \mathcal{A}, r_R + \omega^\prime \log \pi, p).$$ This indicates that we can find the maximum-entropy policy solving the full MDP problem $\hat{\mathcal{M}}$ by solving an augmented MDP problem $\mathcal{M}^\mathrm{aug}$, where $\omega^\prime = \omega \alpha$ is a parameter that balances the optimality between basic and add-on tasks. 

\section{Residual Policy Gradient}\label{sec:RLC-residual_PG}
In this section, we first derive a more neutral form of the maximum-entropy policy gradient methods \textit{Soft Policy Gradients}, which leads to \textit{Residual Policy Gradient} (RPG). Furthermore, we propose \textit{Soft PPO} and \textit{Residual PPO} as two practical algorithms for deployment.

\subsection{Soft Policy Gradient}\label{sec:RLC-SPG}
% Motivation
As discussed in Sec.~\ref{sec:RLC-RQL}, to utilize the augmented MDP problem $\mathcal{M}^\mathrm{aug}$, we need to extend the policy gradient methods to optimize the maximum-entropy policy.

Let $\tau = (\boldsymbol{s}_0, \boldsymbol{a}_0, \boldsymbol{s}_1, \boldsymbol{a}_1, \dots, \boldsymbol{s}_t, \boldsymbol{a}_t, \dots)$ represent a complete trajectory, and $p_\theta(\tau)$ represents the probability density of $\tau$ generated by a parameterized policy $\pi_\theta$ and the environment dynamics $p(\cdot|\boldsymbol{s},\boldsymbol{a})$. The maximum-entropy objective can be written as:
\begin{equation}\label{eqn:MERL_obj}
J(\pi_\theta) = \mathbb{E}_{\tau \sim p_\theta(\tau)}\left[\sum_{t=0} \gamma^t \left(r(\boldsymbol{s}_t,\boldsymbol{a}_t)+\alpha \mathbb{E}_{\boldsymbol{a}_t\sim\pi_\theta(\cdot|\boldsymbol{s}_t)}\left[-\log\pi_\theta\left(\boldsymbol{a}_t|\boldsymbol{s}_t\right)\right]\right)\right].
\end{equation}


The estimation of its gradient $\nabla_\theta J(\pi_\theta)$ can be derived as:
\begin{equation}
\label{eqn:RLC-SPG}
\mathbb{E}_{\tau \sim p_\theta(\tau)} \left[ \sum_{t=0} \nabla_\theta \log \pi_\theta\left(\boldsymbol{a}_t|\boldsymbol{s}_t\right) \left(\sum_{t^\prime = t} \gamma^{t^\prime - t} \left(
    r(\boldsymbol{s}_{t^\prime},\boldsymbol{a}_{t^\prime})-\alpha\log\pi_{\theta}\left(\boldsymbol{a}_{t^\prime}|\boldsymbol{s}_{t^\prime}\right)\right) \right) \right]
\end{equation}

% \begin{equation}
% \mathbb{E}_{\tau \sim p_\theta(\tau)} \left[ \sum_{t=0}
% \nabla_\theta \log \pi_\theta (\boldsymbol{a}_t | \boldsymbol{s}_t) \left( \sum_{t^\prime=t} \gamma^{t^\prime-t} \left(r(\boldsymbol{s}_{t^\prime},\boldsymbol{a}_{t^\prime}) - \alpha\log \pi_\theta(\boldsymbol{a}_{t^\prime} | \boldsymbol{s}_{t^\prime})\right) - V^{\pi_\theta}(\boldsymbol{s}_t) \right)  \right],
% \end{equation}

% where $V^{\pi_\theta}(\boldsymbol{s}_{t}) = \mathbb{E}_{\tau \sim p_\theta(\tau)} \left[\sum_{t^\prime=t} \gamma^{t^\prime-t} \left(r(\boldsymbol{s}_{t^\prime},\boldsymbol{a}_{t^\prime})-\alpha\log\pi_{\theta}\left(\boldsymbol{a}_{t^\prime}|\boldsymbol{s}_{t^\prime}\right)\right)\right]$ is the value function. 
This is equivalent to applying policy gradient over a reformulated reward $r(\boldsymbol{s}_{t},\boldsymbol{a}_{t})-\alpha\log\pi_{\theta}\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)$.
A detailed derivation can be found in Appendix~\ref{appendix:RLC-derivation}. 

\subsubsection{Comparative Analysis of Soft Policy Gradient Derivations} 
Although some previous works \parencite{williams1992simple, mnih2016asynchronous, shi2019soft, schulman2017equivalence} also focused on deriving the maximum-entropy policy gradient, their formulations come with certain inconsistencies or implicit assumptions. With a unified notation, we compare and highlight their similarities and differences.

In the naive entropy regularized policy gradient methods \parencite{williams1992simple, mnih2016asynchronous}, the gradient estimator is encouraged with only an entropy term at the end, which is:
\begin{equation}
\label{eqn:RLC-end-entropy}
\mathbb{E}_{\tau \sim p_\theta(\tau)} \left[ \sum_{t=0}
\nabla_\theta \log \pi_\theta (\boldsymbol{a}_t | \boldsymbol{s}_t) \left( \sum_{t^\prime=t} \gamma^{t^\prime-t} r(\boldsymbol{s}_{t^\prime},\boldsymbol{a}_{t^\prime})
% - V^{\pi_\theta}(\boldsymbol{s}_t) 
\right) - \alpha \nabla_\theta \mathcal{H}\left(\pi_\theta \left(\cdot | \boldsymbol{s}_t\right) \right)  \right].
\end{equation}

Note that $\mathbb{E}_{\tau \sim p_\theta(\tau)} \left[ \sum_{t=0}
\nabla_\theta \mathcal{H}\left(\pi_\theta \left(\cdot | \boldsymbol{s}_t\right) \right) \right] = \mathbb{E}_{\tau \sim p_\theta(\tau)} \left[ \sum_{t} \nabla_\theta \log \pi_\theta(\boldsymbol{a}_t | \boldsymbol{s}_t) \left(\log \pi_\theta(\boldsymbol{a}_t | \boldsymbol{s}_t) \right) \right]$, we can reformulate the naive gradient estimator with a delta function:
\begin{equation}
\begin{aligned}
\mathbb{E}_{\tau \sim p_\theta(\tau)} \left[ \sum_{t=0} 
\nabla_\theta \log \pi_\theta (\boldsymbol{a}_t | \boldsymbol{s}_t) \left( \sum_{t^\prime=t} \gamma^{t^\prime-t} \left(r(\boldsymbol{s}_{t^\prime},\boldsymbol{a}_{t^\prime}) - \alpha \delta(t^\prime, t)\log \pi_\theta(\boldsymbol{a}_{t^\prime} | \boldsymbol{s}_{t^\prime}) \right) 
% - V^{\pi_\theta}(\boldsymbol{s}_t) 
\right)  \right],
\end{aligned}
\end{equation} 
which indicates that the naive methods only consider the first-step ($t^\prime = t$) entropy bonus in updating.


In \cite[Eqn.~(80)]{schulman2017equivalence}, the author introduced the proper entropy bonus on every step to the expected return but retained the $- \alpha \nabla_\theta \mathcal{H}\left(\pi_\theta \left(\cdot | \boldsymbol{s}_t\right) \right)$ term, leading to an update as:
\begin{equation}
\label{eqn:RLC-repeat-entropy}
\mathbb{E}_{\tau \sim p_\theta(\tau)} \left[ \sum_{t=0}
\nabla_\theta \log \pi_\theta (\boldsymbol{a}_t | \boldsymbol{s}_t) \left( \sum_{t^\prime=t} \gamma^{t^\prime-t} \left( r(\boldsymbol{s}_{t^\prime},\boldsymbol{a}_{t^\prime}) - \alpha (\delta(t^\prime, t)+1)\log \pi_\theta(\boldsymbol{a}_{t^\prime} | \boldsymbol{s}_{t^\prime})\right) 
% - V^{\pi_\theta}(\boldsymbol{s}_t) 
\right)  \right],
\end{equation}
which repeats the entropy bonus on the first step.



In \cite[Eqn.~(13)]{shi2019soft}, the derived gradient estimator is
\begin{equation}
\label{eqn:RLC-tsinghua derivation}
    \mathbb{E}_{\tau \sim p_\theta(\tau)} \left[\sum_{t=0} \nabla_\theta \log \pi_\theta\left(\boldsymbol{a}_t|\boldsymbol{s}_t\right) \left(Q^{\pi_\theta}(\boldsymbol{s}_{t},\boldsymbol{a}_{t}) - \alpha\log\pi_{\theta}\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right) - 1 \right)   \right].
\end{equation}
Since     $\mathbb{E}_{\tau \sim p_\theta(\tau)} \left[\sum_{t=0} \nabla_\theta \log \pi_\theta\left(\boldsymbol{a}_t|\boldsymbol{s}_t\right)   \right] = 0$, we can eliminate the $1$ in Eqn.~(\ref{eqn:RLC-tsinghua derivation}) which leads to our result by substituting $Q^{\pi_\theta}(\boldsymbol{s}_{t},\boldsymbol{a}_{t}) = r(\boldsymbol{s}_{t},\boldsymbol{a}_{t}) + \sum_{t^\prime > t} \gamma^{t^\prime-t} \left(
    r(\boldsymbol{s}_{t^\prime},\boldsymbol{a}_{t^\prime})-\alpha\log\pi_{\theta}\left(\boldsymbol{a}_{t^\prime}|\boldsymbol{s}_{t^\prime}\right)\right)$.


\subsection{Practical Algorithm}
\label{sec:RLC- practical algorithm}
\subsubsection{Soft PPO} 
By applying the advantage function, we can reform the gradient:
\begin{equation}\label{eqn:Final_SPG}
    \nabla_\theta J(\pi_\theta) = \mathbb{E}_{\tau \sim p_\theta(\tau)} \left[ \sum_{t=0} \nabla_\theta \log \pi_\theta\left(\boldsymbol{a}_t|\boldsymbol{s}_t\right) A^{\mathrm{SPG}}_{\pi_\theta}(\boldsymbol{s}_t,\boldsymbol{a}_t) \right],
\end{equation}
where
\begin{equation}
    A^{\mathrm{SPG}}_{\pi_\theta}(\boldsymbol{s}_t,\boldsymbol{a}_t) = r(\boldsymbol{s}_{t},\boldsymbol{a}_{t})-\alpha\log\pi_{\theta}\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right) + \gamma \mathbb{E}_{\boldsymbol{s}_{t+1}\sim p(\cdot|\boldsymbol{s}_t,\boldsymbol{a}_t)}  [V^{\pi_\theta}(\boldsymbol{s}_{t+1})] - V^{\pi_\theta}(\boldsymbol{s}_{t}),
\end{equation}
\begin{equation}
    V^{\pi_\theta}(\boldsymbol{s}_{t}) = \mathbb{E}_{\tau \sim p_\theta(\tau)} \left[\sum_{t^\prime=t} \gamma^{t^\prime-t} \left(
    r(\boldsymbol{s}_{t^\prime},\boldsymbol{a}_{t^\prime})-\alpha\log\pi_{\theta}\left(\boldsymbol{a}_{t^\prime}|\boldsymbol{s}_{t^\prime}\right)\right)\right],
\end{equation}
which is equivalent to applying classic policy gradient over $r^{\mathrm{SPG}} = r(\boldsymbol{s}_{t},\boldsymbol{a}_{t})-\alpha\log\pi_{\theta}\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)$.

However, vanilla policy gradient methods have several limitations, such as poor data-efficiency and robustness~\parencite{schulman2017proximal}. To enhance practical performance, we incorporate this reformulated reward into the PPO framework, leading to the Soft PPO method:
\begin{equation}\label{eqn:Soft PPO obj}
\quad \nabla_\theta J(\pi_\theta) = \nabla_\theta \mathbb{E}_{(\boldsymbol{s}_t,\boldsymbol{a}_t)\sim\pi_\theta,p(\cdot|\boldsymbol{s},\boldsymbol{a})} \left[ \min \{r_t(\pi_\theta) A^{\mathrm{SPG}}_{\pi_\theta}, \operatorname{clip}(r_t(\pi_\theta), 1 - \epsilon, 1 + \epsilon) A^{\mathrm{SPG}}_{\pi_\theta} \} \right].
\end{equation}


% Residual PPO
\subsubsection{Residual PPO} 
With the derived Soft Policy Gradient in Sec.~\ref{sec:RLC-SPG}, the residual policy can be obtained by directly applying it on the augmented MDP $\mathcal{M}^{\mathrm{aug}}=(\mathcal{S}, \mathcal{A}, r_R + \omega'\log\pi,p)$:
\begin{equation}
% \label{eqn:Soft PPO obj}
\quad \nabla_\theta J(\pi_\theta) = \nabla_\theta \mathbb{E}_{(\boldsymbol{s}_t,\boldsymbol{a}_t)\sim\pi_\theta,p(\cdot|\boldsymbol{s},\boldsymbol{a})} \left[ \min \{r_t(\pi_\theta) A^{\mathrm{RPG}}_{\pi_\theta}, \operatorname{clip}(r_t(\pi_\theta), 1 - \epsilon, 1 + \epsilon) A^{\mathrm{RPG}}_{\pi_\theta} \} \right].
\end{equation}
where $A^{\mathrm{RPG}}_t$ is estimator of the advantage over the reformulated reward $r^{\mathrm{RPG}}$ at timestep $t$:




\begin{equation}
\label{eqn:RLC-RPG Reward}
r^{\mathrm{RPG}}(\boldsymbol{s}_{t},\boldsymbol{a}_{t}) = 
r_R(\boldsymbol{s}_{t},\boldsymbol{a}_{t}) 
+\omega^\prime \log  {\pi\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)} 
- \hat{\alpha} \log {{\pi_{\theta}\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)}}.
% = r(\boldsymbol{s}_{t},\boldsymbol{a}_{t}) + \beta \log{\pi\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)}- \beta \log {{\pi_{\theta}\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)}}
\end{equation}

Building upon the widely used "End-Entropy PPO" (\cite{mnih2016asynchronous}, Eqn.~(\ref{eqn:RLC-end-entropy})), our method only requires adding the corresponding $- \hat{\alpha} \log {{\pi_{\theta}\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)}}$ and $\omega^\prime \log  {\pi\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)}$ when computing the advantage, and removes the repeat term $- \alpha \nabla_\theta \mathcal{H}\left(\pi_\theta \left(\cdot | \boldsymbol{s}_t\right) \right)$ when computing the actor loss, to obtain Soft PPO or Residual PPO, which makes it easily deployable within established PPO pipelines.

% \newpage
\subsection{A Reward View of KL-regularized Objective}


\subsubsection{Not Just a KL-regularized Objective}
\label{sec:RLC- KL-constrained Reward}
The use of KL objective can be traced back to KL Control~\parencite{todorov2006linearly}, which is a branch of stochastic optimal control, and was later introduced into RL~\parencite{fox2015taming, rawlik2013stochastic, jaques2017sequence}. The maximized objective follows the form~\parencite[Eqn.~(2)]{jaques2017sequence}:

\begin{equation}
\label{eqn:RLC-KL Objective}
\mathbb{E}_{\pi_\theta} \left[ \sum_{t' = t}^{\infty} r_R(\boldsymbol{s}_{t^\prime}, \boldsymbol{a}_{t^\prime}) + \beta \log\frac{ \pi(\boldsymbol{a}_{t^\prime}|\boldsymbol{s}_{t^\prime})}{ \pi_\theta(\boldsymbol{a}_{t^\prime}|\boldsymbol{s}_{t^\prime})} \right],
\end{equation}

% Reward Interpretation
which aligns with the form of maximum-entropy RL objective in Eqn.~(\ref{eqn:MERL_obj}) by taking $r = r_R + \log \pi$. Following the derivation in Sec.~\ref{sec:RLC-SPG} and Sec.~\ref{sec:RLC- practical algorithm}, this form could be view as a special case of RPG whose advantage is calculated on reward:
\begin{equation}
\label{eqn:RLC-KL Reward}
r^{\text{KL}}(\boldsymbol{s}_{t},\boldsymbol{a}_{t}) = 
r_R(\boldsymbol{s}_{t},\boldsymbol{a}_{t}) 
+\beta \log  {\pi\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)} 
- \beta \log {{\pi_{\theta}\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)}}.
% = r(\boldsymbol{s}_{t},\boldsymbol{a}_{t}) + \beta \log{\pi\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)}- \beta \log {{\pi_{\theta}\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)}}
\end{equation}

Similarly, in Eqn.~
(\ref{eqn:RLC-RPG Reward}), the decomposed KL divergence can be viewed as a combination of an augmentation reward $\beta \log \pi$ and an entropy-encouragement term $\beta \log \pi_\theta$. Specifically, if we further assume that prior policy $\pi$ is a maximum-entropy policy encouraged by the same entropy coefficient of the customized policy $\alpha = \beta$, and the optimizing objective is the direct sum of the implicit reward and the preference reward $\omega = 1$, then the KL-regularized objective actually leads to a maximum-entropy policy on a MDP:

\begin{equation}
\label{eqn:RLC-KL MDP}
    \mathcal{M}^\mathrm{KL} = (\mathcal{S}, \mathcal{A}, r + r_R, p).
\end{equation}

This decoupling reveals that the KL-constrained reward has a theoretical foundation beyond its simple intuition to just prevent the fine-tuned model from drifting too far from the pretrained model. That is, it is optimizing a trade-off between basic and add-on tasks on the reward level.

% $r_R(\boldsymbol{s}_{t},\boldsymbol{a}_{t})$ is the add-on reward, $\beta \log \pi$ provided by the prior policy represents the augmented reward, and $\beta \log \pi_\theta$ is the entropy-encouraging term. 



% Moreover, it can be seen as a special case of the proposed RPG reward with $\omega = 1$ and $\alpha = \hat{\alpha} = \beta$.
% explanation
% This implies that Vanilla RLHF is actually optimizing on the equal sum of the implicit reward of human language and a preference reward $r_{\mathrm{human}} + r_R$ ($\omega = 1$), while encouraging the entropy to the same extent ($\alpha = \hat{\alpha}$), or simply:




% Moreover, by assuming that the original LLM was trained under the maximum-entropy principle, this update rule indicates that the RLHF optimizes on a latent full MDP problem $\hat{\mathcal{M}}^\mathrm{RLHF} = (\mathcal{X}, \mathcal{U}, r_{\pi} + r, p)$, where $ r_{\pi}$ is the latent reward the original LLM optimized on.





\subsubsection{Not Necessarily a KL-regularized Objective}
\label{sec:RLC- More than KL-constrained Reward}
However, according to the derivation of RPG, such reward reparameterization is not limited to being implemented via KL divergence but can instead be decoupled into two tunable parameters $\omega^\prime$ and $\hat{\alpha}$ as in Eqn.~(\ref{eqn:RLC-RPG Reward}):
$r^{\mathrm{RPG}}(\boldsymbol{s}_{t},\boldsymbol{a}_{t}) = 
r_R(\boldsymbol{s}_{t},\boldsymbol{a}_{t}) 
+\omega^\prime \log  {\pi\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)} 
- \hat{\alpha} \log {{\pi_{\theta}\left(\boldsymbol{a}_{t}|\boldsymbol{s}_{t}\right)}}$.

In practice, the prior policy does not necessarily follow the maximum-entropy property, nor is it necessarily optimal. 
Meanwhile, the entropy-encouragement coefficient of the prior policy may not be accessible, and the newly trained policy does not necessarily need to maintain the same entropy coefficient.
This flexibility enables fine-tuning without strictly relying on the KL-regularized objective, allowing for a more adaptable approach. 
In the next section, we empirically validate this perspective through experiments by comparing Residual PPO and classic KL-regularized PPO.

In Appendix~\ref{appendix:RLC-RLHF}, taking Reinforcement Learning for LLM fine-tuning as an example, we demonstrate how the insights in Sec.~\ref{sec:RLC- KL-constrained Reward} and Sec.~\ref{sec:RLC- More than KL-constrained Reward} deepen our understanding and informs future directions.

\section{Experiments}

\subsection{Soft PPO}
% \subsubsection{Setting}
\label{sec:RLC- Soft PPO}
In this section, we evaluate the preliminary algorithm, Soft PPO, across several continuous control benchmarks in MuJoCo. 

\textbf{Baselines.} We select the variants mentioned in Sec~\ref{sec:RLC-SPG} as baselines:
\begin{itemize}[leftmargin=20pt]

\item[-] \textbf{No-Entropy PPO:}
First, we evaluate the classic PPO without entropy term, serving as a baseline performance compared to entropy-regularized approaches.

\item[-] \textbf{End-Entropy PPO:}
Next, we evaluate the form of Eqn.~(\ref{eqn:RLC-end-entropy}) \parencite{williams1992simple, mnih2016asynchronous}, which only considers the entropy of the first step. By comparing against this baseline, we investigate whether introducing the entropy term at each step enhances exploration effectiveness.

\item[-] \textbf{Repeat-Entropy PPO:}
Finally, we evaluate the form of Eqn.~(\ref{eqn:RLC-repeat-entropy}) \parencite{schulman2017equivalence}, which repeats the entropy of the first step. By comparing against this baseline, we investigate whether removing the repeated entropy term leads to performance improvements.

\end{itemize}

% std design
When modeling the policy distribution, we adopted the common implementation approach in PPO~\parencite{mnih2016asynchronous}, using a global standard deviation instead of a state-dependent one. While this reduces the policy interpretability, it improves practical performance by simplifying learning and enhancing stability. A detailed ablation can be found in  appendix~\ref{sec:RLC-appendix-Implementation-mujoco}.

% Table Results

\begin{table}[t]
\caption{\textbf{Experimental Results of Entropy-Regularized PPO Variants in MuJoCo.} The evaluation results are over 500 episodes across 5 seeds, and in the form of $\mathrm{mean} \pm \mathrm{std}$.}
\label{tbl:RLC-Soft PPO Results}
\resizebox{\textwidth}{!}{
\begin{threeparttable}
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{5}{c}{Average Performance} \\
\midrule
\multirow{1}{*}{Env.} & No-Entropy PPO & End-Entropy PPO & Repeat-Entropy PPO & Soft PPO\\ \midrule
Ant          & $3918.9 \pm 1032.9$ & $3887.9 \pm 991.4$ & $3241.2 \pm 1299.7$ & $\mathbf{3845.6 \pm 911.7}$  \\
Hopper       & $2387.3 \pm 1060.6$ & $2696.3 \pm 978.0$ & $2611.6 \pm 967.8$ & $\mathbf{3105.3 \pm 829.5}$  \\
Half Cheetah & $2254.9 \pm 1188.7$ & $3291.5 \pm 2006.0$ & $-114.9 \pm 73.2$ & $\mathbf{4993.7\pm 1262.3}$  \\
\midrule
\multicolumn{5}{c}{Best Performance} \\
\midrule
\multirow{1}{*}{Env.} & No-Entropy PPO & End-Entropy PPO & Repeat-Entropy PPO & Soft PPO\\ \midrule
Ant          & $4389.6 \pm 296.7$ & $4223.4 \pm 822.6$ & $4023.9 \pm 786.3$ & $4581.1 \pm 540.3$  \\
Hopper       & $3271.2 \pm 573.4$ & $3654.4 \pm 46.4$ & $3404.2 \pm 226.0$ & $3689.4 \pm 29.2$  \\
Half Cheetah & $4136.6 \pm 1566.6$ & $6049.3 \pm 946.2$ & $-38.9 \pm 58.2$ & $5896.5\pm 371.8$  \\


\bottomrule

\vspace{-3em} 
\end{tabular}

\end{threeparttable}
}
\end{table}





% \subsubsection{Results}
\textbf{Does the proposed formulation achieve empirical performance improvements?}
As shown in Table~\ref{tbl:RLC-Soft PPO Results}, compared to other variants of entropy-encouraged PPO, the proposed Soft PPO exhibits comparable or potentially better average performance. 
Specifically, in the HalfCheetah task, we observed significant performance differences among variants with different entropy encouragement. This indicates that PPO can be very sensitive to the way to encourage entropy-regularized learning: although Repeat-Entropy PPO shares the same parameters and similar updating mechanism with Soft PPO, they can behave completely differently during learning.

Notably, the best-performing seeds in the compared variants achieve similar performance to Soft PPO, 
whose overall performance declines are generally due to more seeds converging to the local sub-optimal.
This further indicates that the concise formulation of Soft PPO can potentially better encourage the agent to explore the environment effectively. However, it is also worth noting that since End-Entropy PPO considers entropy encouragement in fundamentally different ways compared to Repeat-Entropy PPO and Soft PPO, they adopt different entropy coefficients, which remains room for better performance with more fine-grained tuning. In practical applications, we consider all these variants to be selectable based on the specific characteristics of the problem.

% \textcolor{entropy-regularized scale issue}

% CPPO Issue
% In PPO, there is a significant issue for practical deployment: even methods that rely on the entropy regularization term often choose, in actual implementation, to set the policy’s standard deviation as a tunable parameter that is independent of the current state and uniform across all actions.


% This assumption leads the log-pi term to reflect less prior policy information, potentially causing performance deterioration in both Soft Policy Learning and Residual Learning. On the other hand, accurately modeling a proper distribution remains a challenging problem in learning, which can likely result in training instability and performance losses under limited computational budget


\subsection{Residual PPO}

% \subsubsection{Setting}

In this section, we evaluate the proposed Residual PPO in the same MuJoCo environments but with extra add-on rewards, which are designed to illustrate customized specifications during practical deployments~\parencite{ResidualMPPI}. 
In HalfCheetah, an add-on penalty on the angle of a certain joint is applied to simulate a common issue in deployment when the corresponding motor is broken. 
In Hopper and Ant, the extra rewards are assigned on height and velocity for moving along the y-axis. 
The configurations of environments and training can be found in Appendix~\ref{appendix:RLC-environment configuration} and Appendix~\ref{appendix:RLC-implementation setting}.

% Metric
\textbf{Metrics.} We evaluate a policy's performance with the total reward $R = r+r_R$, since it represents the objective of the policy customization task. However, when the add-on task conflicts with the basic task, the optimal policy may sacrifice performance on the basic task to maximize the total reward. To better monitor this trade-off during customization, we separately measure the basic and add-on rewards, allowing us to assess how well the customized policy preserves the basic task's performance while optimizing for the add-on task ~\parencite{ResidualMPPI}.

% Baselines: Prior/ Residual-MPPI/ Full-MPPI/ Guided-MPPI
\textbf{Baselines.} In our experiments, we mainly compare Residual PPO against four baselines:

\begin{itemize}[leftmargin=20pt]

\item[-] \textbf{Prior Policy:}
First, we evaluate the best-performing Soft PPO checkpoint in Sec.~\ref{sec:RLC- Soft PPO} on the full task, which serves as a baseline to show the effectiveness of policy customization.

\item[-] \textbf{Greedy PPO:}
Next, we finetune the prior policy towards the add-on reward solely, which can be achieved by setting $\omega^\prime=0$, which serves as a trivial baseline when basic reward is unknown.

\item[-] \textbf{KL PPO:}
Next, we utilize the KL divergence to regularize the fine-tuning process, which can be achieved by setting $\omega^\prime=\hat{\alpha}$, which serves as a widely-used practical fine-tuning baseline.

\item[-] \textbf{Full Policy:}
Finally, we utilize the Soft PPO to train an optimal policy on the full task, which serves as an upper-bound performance of policy customization 

\end{itemize}


% \subsubsection{Results}

\begin{table}[t]
\caption{\textbf{Experimental Results of Residual PPO in MuJoCo.} The evaluation results are over 500 episodes with best-performing checkpoints across 5 seeds. The results are in the form of $\mathrm{mean} \pm \mathrm{std}$.} 
\label{tbl:RLC-Customization Results}

\resizebox{\textwidth}{!}{

\begin{threeparttable}
\begin{tabular}{@{}clcccc@{}}
\toprule
\multirow{2}{*}{Env.} & \multicolumn{1}{c}{\multirow{2}{*}{Policy}} & Full Task  & {Basic Task} & \multicolumn{2}{c}{Add-on Task} \\ \cmidrule(l){3-6}
 & & $\mathrm{Total\ Reward}$ & $\mathrm{Basic\ Reward}$ &  $\bar{|\theta|}$ & $\mathrm{Add}$-$\mathrm{on\ Reward}$ \\
 \midrule
 
\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Half\\ Cheetah\end{tabular}} 
& Prior Policy  & $5357.0 \pm 377.8$            & $5896.5 \pm 371.8$   & $0.54 \pm 0.01$                &  $-539.8 \pm 8.7$                 \\
\cmidrule(l){2-6} 
& Greedy PPO    & $-1314.0 \pm 252.4$           & $-1150.2 \pm 236.0$  & $0.16 \pm 0.02$                &  $-163.7 \pm 21.8$                \\
& KL PPO        & $5418.7 \pm 150.1$            & $5776.3 \pm 133.7$   & $0.36 \pm 0.02$                &  $-357.6 \pm 17.7$                \\ 
& Residual PPO  & $\mathbf{5488.3 \pm 75.6}$    & $5845.1 \pm 69.5$    & $\mathbf{0.36 \pm 0.01}$       &  $\mathbf{-356.3 \pm 8.6}$        \\
\cmidrule(l){2-6} 
& Full Policy   & $5556.2 \pm 57.8$             & $6011.4 \pm 57.2$    & $0.46 \pm 0.01$                &  $-455.2 \pm 5.8$                 \\
\midrule 
 
\multicolumn{1}{c}{Env} & \multicolumn{1}{c}{Policy} & $\mathrm{Total\ Reward}$ & $\mathrm{Basic\ Reward}$ & $\bar{z}$ & $\mathrm{Add}$-$\mathrm{on\ Reward}$ \\
\midrule
\multirow{5}{*}{Hopper} 
& Prior Policy      & $5133.7 \pm 33.2$             & $3689.4 \pm 29.2$    & $1.44 \pm 0.01$          &  $1444.3 \pm 6.0$             \\
\cmidrule(l){2-6} 
& Greedy PPO        & $3714.5 \pm 7.1$              & $2224.2 \pm 6.5$     & $1.49 \pm 0.00$            &  $1490.2 \pm 0.9$             \\
& KL PPO            & $3864.4 \pm 50.10$            & $2400.3 \pm 55.2$    & $1.46 \pm 0.01$            &  $1464.1\pm 6.1$              \\ 
& Residual PPO      & $\mathbf{4401.4 \pm 505.3}$   & $2951.6 \pm 333.5$   & $\mathbf{1.50 \pm 0.03}$   &  $\mathbf{1449.5 \pm 177.0}$  \\
\cmidrule(l){2-6} 
& Full Policy       & $5142.7 \pm 34.8$             & $3669.0 \pm 26.8$    & $1.47 \pm 0.00$            &  $1473.6 \pm 8.4$             \\
\midrule      
                           
\multicolumn{1}{c}{Env.} & \multicolumn{1}{c}{Policy} & $\mathrm{Total\ Reward}$ & $\mathrm{Basic\ Reward}$ & $\bar{v}_y$ & $\mathrm{Add}$-$\mathrm{on\ Reward}$ \\
\midrule
\multirow{5}{*}{Ant} 
& Prior Policy      & $4875.2 \pm 589.4$            & $4581.1 \pm 540.3$   & $0.29 \pm 0.13$            &  $294.1 \pm 133.9$             \\
\cmidrule(l){2-6} 
& Greedy PPO        & $4340.6 \pm 1464.5$           & $726.4 \pm 277.1$    & $3.86 \pm 0.96$            &  $3613.9 \pm 1246.4$           \\ 
& KL PPO            & $4019.4 \pm 1103.4$           & $368.6 \pm 151.8$    & $3.74 \pm 0.92$            &  $3650.6 \pm 1047.6$           \\ 
& Residual PPO      & $\mathbf{5568.3 \pm 852.4}$   & $1340.8 \pm 220.0$   & $\mathbf{4.27 \pm 0.63}$   &  $\mathbf{4227.4 \pm 705.3}$   \\
\cmidrule(l){2-6} 
& Full Policy       & $6185.1 \pm 1142.0$           & $3543.0 \pm 621.2$   & $2.70 \pm 0.41$            &  $2641.6 \pm 542.8$            \\
\bottomrule

\end{tabular}
    % \begin{tablenotes}
    %     \small
    %     \item 
    % \end{tablenotes}
\end{threeparttable}
}
% \vspace{-2em}
\end{table}




\textbf{Can Residual PPO effectively solve the policy customization problem?}
The experimental results, summarized in Table~\ref{tbl:RLC-Customization Results}, demonstrate the effectiveness of Residual PPO for policy customization. 
% Add-on Task Improvements
Across all tasks, Residual PPO achieves obvious performance improvements on the add-on task compared to the prior policy, demonstrating its capability to optimize the prior policy for new requirements. 
Moreover, in the HalfCheetah and Ant, Residual PPO achieves performance comparable to the performance of the Full Policy, which indicates that by incorporating the $\log \pi$, Residual PPO can effectively balance the trade-off between the basic and the add-on task.

\textbf{Does the flexibility of decoupling lead to more effective policy customization?}
Greedy PPO, due to optimizing towards the add-on reward solely, struggles to maintain its performance on the basic task, resulting in a lower total reward compared to Residual PPO. 
This issue becomes more pronounced in tasks requiring auxiliary rewards, such as action regularization, where Greedy PPO fails to train an effective policy in the HalfCheetah task. 
KL PPO, in theory, should achieve the best performance as it optimizes a MDP with the exact objective $R = r+r_R$ and a reasonable entropy coefficient $\hat{\alpha} = \alpha$. However, as discussed in Sec.~\ref{sec:RLC- More than KL-constrained Reward}, the maximum-entropy and optimality assumptions of RPG do not hold in practical scenarios, which can lead to even worse performance, as shown in Ant results.
% Emphasis on Flexibility
In contrast, the decoupling of the KL-regularized term in RPG provides greater tuning flexibility, which can lead to superior performance in practical applications.
% Limitation
However, when this flexibility encounters excessively large assumption misalignments, it can also lead to suboptimal customization results, as observed in the Hopper task.
% Limitation and Future work
This also suggests that when building a foundation model that is more adaptable, adequate modeling of complex distributions is an important direction for future work.







\section{Related Work}\label{sec:RLC-related-work}

\textbf{KL-regularized Objective.}
The KL-regularized objective is related to KL Control~\parencite{todorov2006linearly, kappen2012optimal}, which aims to prevent the target policy from deviating too far from a reference, which is widely adopted in RL. $\Psi$-learning~\parencite{rawlik2013stochastic} and G-learning~\parencite{fox2015taming} both maximize the reward while incurring penalties for the KL-divergence from reference policies.
% RL-Finetuning
The KL-regularized objective is also a common approach in transfer learning~\parencite{tirumala2019exploiting} and RL-based finetuning~\parencite{nair2020awac}, especially for fine-tuning LLM with human preference. Using RL for LLM fine-tuning as an example, we provide a detailed discussion in Appendix~\ref{appendix:RLC-RLHF}.

The flexibility of KL decoupling discussed in Sec.~\ref{sec:RLC- More than KL-constrained Reward} can be achieved through alternative approaches. Distral~\parencite{teh2017distral} simultaneously employs KL divergence and entropy with different coefficients to regularize the joint training of the task-specific and meta policy. TD-M(PC)\textsuperscript{2}~\parencite{lin2025td}
uses the log distribution to bring the nominal policy and planner closer during learning, leading to a more higher-performing policy.
However, these results are derived from practical usage, whereas RPG provides a reward-level perspective to support such implementations.



% \subsection{Residual Q-Learning}
\textbf{Residual Q-Learning.} 
% RQL introduction again
RQL~\parencite{RQL} proposes a principled framework to solve policy customization without the reward knowledge of the prior policy. 
% Extension
However, this framework is not limited to RL-based approaches or policy customization alone: inspired by RQL, Residual-MPPI~\parencite{ResidualMPPI} integrates model-based planning to enable online policy customization, while MEReQ~\parencite{MEREQ} leverages RQL as an efficient approach for inverse RL.

% Alike Work
Many works originating from preference-based RL have ultimately derived results similar to RQL, and converge toward maximum-entropy RL, specifically the $\log \pi$ form. IQ-Learn~\parencite{garg2021iq} and IPL~\parencite{hejna2024inverse}  all recognized that learning the maximum-entropy policy or Q-value provides an implicit yet efficient way to capture preferences from data, leading to an updating approach similar to RQL. However, these methods focus on Inverse RL, whereas RQL directly formulates a training pipeline from the perspective of optimizing a new policy, 


% \subsection{Model as Reward}
% \textbf{Model as Reward.} 
% % More General Way
% The core of RQL-inspired $\mathcal{M}^\mathrm{aug}$ is utilizing the learned policy as a reward function. This idea has been reflected in many recent works.
% % Introduction
% Beyond the works~\parencite{yuan2024implicitprm, rafailov2024direct, rafailov2024r} mentioned in Section~\ref{sec:RLC- RQL View}, many other methods focus on a high-level or intuition-driven approach to achieve this goal. 
% % LLM as reward
% \textcite{kwon2023reward} first proposed that LLM can work as a reward generator in text-based RL environments. Constitutional AI~\parencite{bai2022constitutional} mix preference labels generated by LLMs and humans during the RLHF process.
% % RL-VLM-F: Use VLM as a Labeler
% Furthermore, RL-VLM-F~\parencite{wang2024rl} completely replaces human annotators with a VLM to provide preference labels, thus learning a specific reward function.
% % However
% However, despite their practical success, the intuition-driven nature of these methods prevents a deeper insight into what these approaches are actually optimizing.



\section{Conclusion}\label{sec:RLC-conclusion}
% Derivation
In this chapter, we derived a concise form of the maximum-entropy policy gradient and, based on this foundation, developed the \emph{Residual Policy Gradient} as an important complement to RQL. 
% Experiments
With MuJoCo experiments, we validated the theoretical correctness of the proposed algorithms.
% KL-Reward
Moreover, RPG reveals that the KL-constrained reward has a theoretical foundation beyond its simple intuition.
% RLHF
This enables us to establish clear connections between many successful RLHF methods and further explain certain experimental phenomena observed in them.
% Future
The success of these works also serves as a strong empirical validation for our theoretical framework, laying a solid foundation for future RLHF and broader policy customization research.


